Interpretable Deep Learning for Forecasting Online Advertising Costs: Insights from the Competitive Bidding Landscape

As advertisers increasingly shift their budgets toward digital advertising, accurately forecasting advertising costs becomes essential for optimizing marketing campaign returns. This paper presents a comprehensive study that employs various time-series forecasting methods to predict daily average CPC in the online advertising market. We evaluate the performance of statistical models, machine learning techniques, and deep learning approaches, including the Temporal Fusion Transformer (TFT). Our findings reveal that incorporating multivariate models, enriched with covariates derived from competitors' CPC patterns through time-series clustering, significantly improves forecasting accuracy. We interpret the results by analyzing feature importance and temporal attention, demonstrating how the models leverage both the advertiser's data and insights from the competitive landscape. Additionally, our method proves robust during major market shifts, such as the COVID-19 pandemic, consistently outperforming models that rely solely on individual advertisers' data. This study introduces a scalable technique for selecting relevant covariates from a broad pool of advertisers, offering more accurate long-term forecasts and strategic insights into budget allocation and competitive dynamics in digital advertising.

==> section/appendices.tex <==
\begin{sidewaystable}%[!htb]
{\renewcommand{\arraystretch}{1.5} % padding
    \begin{tabular}{p{3cm}p{0.02cm}p{1cm}p{1cm}p{1.2cm}p{0.02cm}p{1cm}p{1cm}p{1.2cm}p{0.02cm}p{1cm}p{1cm}p{1.2cm}}
    \hline
    \textbf{Model} & & & \textbf{14 days} & & & & \textbf{30 days} & & & & \textbf{60 days} & \\
    & & MAE $\downarrow$ & MAPE $\downarrow$ & SMAPE $\downarrow$ & & MAE $\downarrow$ & MAPE $\downarrow$ & SMAPE $\downarrow$ & & MAE $\downarrow$ & MAPE $\downarrow$ & SMAPE $\downarrow$ \\
    \cline{1-1}
    \cline{3-5}
    \cline{7-9}
    \cline{11-13}
        SARIMA.univar & & 0.211 & \textbf{0.184} & 0.179 & & 0.227 & 0.209 & 0.197 & & 0.306 & 0.299 & 0.264 \\
        \vspace{1pt} \\
        XGB.univar & & 0.259 & 0.241 & 0.225 & & 0.278 & 0.262 & 0.243 & & 0.340 & 0.313 & 0.279 \\
        XGB.multivar & & 0.242 & 0.241 & 0.218 & & 0.271 & 0.233 & 0.231 & & 0.274 & 0.282 & 0.258 \\
        XGB.multivar.comp.cat & & 0.245 & 0.227 & 0.219 & & 0.250 & 0.245 & 0.218 & & 0.278 & 0.270 & 0.423 \\
        XGB.multivar.comp.extr & & 0.248 & 0.232 & 0.228 & & 0.257 & 0.242 & 0.216 & & 0.267 & 0.268 & 0.239 \\
        XGB.multivar.comp.dist & & 0.244 & 0.221 & 0.213 & & 0.246 & 0.230 & 0.227 & & 0.276 & 0.263 & 0.235 \\
        \vspace{1pt} \\
        LSTM.univar & & 0.245 & 0.224 & 0.203 & & 0.265 & 0.243 & 0.217 & & 0.318 & 0.287 & 0.251 \\
        LSTM.multivar & & 0.235 & 0.210 & 0.204 & & 0.250 & 0.221 & 0.215 & & 0.252 & 0.253 & 0.236 \\
        LSTM.multivar.comp.cat & & 0.231 & 0.203 & 0.199 & & 0.229 & 0.223 & 0.202 & & 0.253 & 0.233 & 0.228 \\
        LSTM.multivar.comp.extr & & 0.227 & 0.198 & 0.202 & & 0.235 & 0.224 & 0.199 & & 0.253 & 0.244 & 0.237 \\
        LSTM.multivar.comp.dist & & 0.229 & 0.220 & 0.196 & & 0.231 & 0.219 & 0.210 & & 0.250 & 0.236 & 0.232 \\
        \vspace{1pt} \\
        TFT.univar & & 0.216 & 0.197 & 0.185 & & 0.236 & 0.218 & 0.204 & & 0.307 & 0.274 & 0.241 \\
        TFT.multivar & & 0.203 & 0.192 & 0.180 & & 0.223 & 0.203 & 0.192 & & 0.241 & 0.229 & 0.214 \\
        TFT.multivar.comp.cat & & 0.208 & 0.190 & 0.181 & & 0.215 & 0.196 & 0.188 & & 0.238 & 0.223 & 0.204 \\
        TFT.multivar.comp.extr & & 0.207 & 0.191 & 0.181 & & \textbf{0.211} & 0.199 & 0.186 & & 0.235 & 0.219 & 0.202 \\
        TFT.multivar.comp.dist & & \textbf{0.201} & 0.187 & \textbf{0.177} & & 0.216 & \textbf{0.192} & \textbf{0.183} & & \textbf{0.232} & \textbf{0.210} & \textbf{0.196} \\
    \hline
    \end{tabular}
}
\caption{Model performance comparison of all model and clustering configurations in three forecasting horizons (14 days, 30 days and 60 days)}
\label{table_results}
\end{sidewaystable}

==> section/business_implications.tex <==
There are many important takeaways for practitioners on a modeling and strategic level. First, the model's performance and variable importance analysis show that feeding the model competitor's behavior can dramatically increase its accuracy. Modern data providers make this possible for players of varying sizes within their respective industries. But even more importantly, the model has shown that CPC predictions can highly benefit from budget analysis within the company itself. Classical CPC values are either given last month's data or forecasts on CPC itself - but to see the effect of an advertiser's own budget adjustments on the predicted CPC gives a much broader picture. Allocating budgets over the year, reacting to external shocks of extreme or no demand, and gauging the effect of one spending on the CPC that your competitors will have to pay for, as well as give practitioners a much more potent tool to optimize their ad spend strategy.

An additional finding shows that advertisers should not only look at their direct competitors but identify advertisers with a high correlation to their data, as shown by the time series clustering techniques. An ice cream shop should look at the competitors just as much as a BBQ-grill shop - their highly correlated demand and connected CPC can give models an additional edge.

==> section/related_work.tex <==
\cite{Elsayed2021} 
\cite{Masini2021}


\subsection{Online advertising cost}
Online advertising is gaining more and more importance by providing more efficient methods for advertisers to direct their campaigns towards specific target groups. Intermediary platforms provided by large technology players, such as Google or Facebook, enable matching of ads to customers on a level of individuality that traditional advertising channels can not imitate.





\subsection{Deep learning for time-series forecasting}
